IoT or NoT: Identifying IoT Devices in a ShortTime Scale

In recent years the number of IoT devices in home networks has increased dramatically. Whenever a new device connects to the network, it must be quickly managed and secured using the relevant security mechanism or QoS policy. Thus a key challenge is to distinguish between IoT and NoT devices in a matter of minutes. Unfortunately, there is no clear indication of whether a device in a network is an IoT. In this paper, we propose different classifiers that identify a device as IoT or non-IoT, in a short time scale, and with high accuracy. Our classifiers were constructed using machine learning techniques on a seen (training) dataset and were tested on an unseen (test) dataset. They successfully classified devices that were not in the seen dataset with accuracy above 95%. The first classifier is a logistic regression classifier based on traffic features. The second classifier is based on features we retrieve from DHCP packets. Finally, we present a unified classifier that leverages the advantages of the other two classifiers. We focus on the home-network environment, but our classifiers are also applicable to enterprise networks.

==> sections/Analyzing.tex <==
\section{Analyzing trivial methods}

\subsection{MAC OUI}
A trivial approach based on metadata MAC OUI (organizationally unique identifier, known as manufacturer id) is very limited due to manufacturers that supplies IoT and non-IoT device types (like Samsung's smart cam and Samsung's smartphones) and for manufacturers that supplies generic multiple-purpose chipset.

\subsection{DHCP}
When talking about device identification, DHCP is the most intuitive protocol that comes in mind. 

A method based DHCP hostname can help in some of the cases, where hostname is defined (on many IoT devices the hostname is not configured). However, in some cases hostname value can be misleading due to its easy to change by the users. Moreover, the availability of DHCP packets is too inferior. DHCP packet are very rare, and available only when a device connects to the network or renewing its IP. Also, DHCP packets are only visible on LAN environment. Besides, DHCP packets are not available on static-IP networks. Therefore, it is not available in all scenarios.

\begin{figure}[t]
\centering
\psfig{file=figures/DHCP.png,width=3.5in,}
\caption{Percentage of slots that contains DHCP packets} \label{fig:DHCP}

\end{figure}

\begin{figure}[t]
\centering
\psfig{file=figures/DHCP_diffs.png,width=3.5in,}
\caption{Interleaving time distribution of DHCP packets} \label{fig:DHCP_diffs}
\end{figure}

We made an analysis for how frequent DHCP packets are. Figure shows the presence of DHCP packets in various width's slots. The median for seeing a DHCP packet is about 3 hours.
However, while using active measures, one can retrieve this data instantly. We suggest two methods to achieve this. 1- flash disconnection of all devices; this action causes every device to renegotiate and triggers DHCP traffic. 2- with tr-69 permissions, an ISP level classifier can query each CPE gateway for the required DHCP values of each currently connected device.
In section \ref{classifying_using_dhcp} we suggest a method to classify devices using DHCP data.

\subsection{HTTP User Agent}

\ignore{HAIM: BUT WHAT IS THE INDICATOR OF IoT IN USER AGENT ???; ANAT: I talk about the UA-len in the next section}
User agent is a field that mostly being send during HTTP requests. This field contains a short description of the requesting device. We expect that a description of IoT devices will be notably different from a description of NoT devices.
We made an analysis for how frequent HTTP requests are. Figure shows the presence of HTTP requests in various width's slots, when figure shows the interleaving time distribution between HTTP requests. The median for seeing a HTTP request from an IoT device is about 2 hours. Note that 48 \% from our IoT devices did not use HTTP or send User-Agent data.

\begin{figure}[t]
\centering
\psfig{file=figures/UA_per.png,width=3.5in,}
\caption{Percentage of slots that contains User-Agent field} \label{fig:UA_per}
\end{figure}

\begin{figure}[t]
\centering
\psfig{file=figures/UA_diffs.png,width=3.5in,}
\caption{Interleaving time distribution of packets with User-Agent field} \label{fig:UA_diffs}
\end{figure}


%In Table \ref{tab:features}

==> sections/DHCP.tex <==

\section{DHCP Signature based Classifier}

%\subsubsection{DHCP}

When talking about device identification, DHCP is the most intuitive protocol that comes to mind. In DHCP, the devices use this protocol to notify (usually) the router of their existence in the network.
To classify devices using DHCP, we collect three values: hostname, vendor-class ID (VCI) and parameter request list (PRL). The hostname is the device's name, and it usually contains a value configured by the vendor. However, this value can be changed by the user. The vendor-class ID identifies the device's DHCP client program. The parameter-request-list is a list of parameters the host ask from the DHCP-server to supply upon connection setup. In DHCP supplying these values is optional. Figure \ref{fig:dhcp_vals} illustrates these values in a packet. Analyzing our seen dataset, we found that all devices send at least one value.

\ignore{Analyzing our seen dataset, we found that 4 devices (8.7\%) did not send any of these values. However, as we show later, this usually indicates that the device is an IoT. }

DHCP has a few drawbacks.
First, DHCP packets are only visible in LAN environments, and they are not available in certain network configurations such as static-IP and in some IPv6 networks due to SLAAC (stateless address auto-configuration \cite{rfc4862}).
Second, classification requires the use of DPI, which is costly in terms of CPU.
Third, DHCP packets are rarely available, since DHCP traffic occurs when a device connects to the network or renews its IP.  Figure \ref{fig:DHCP} shows the presence of DHCP packets in slots of various widths. Figure \ref{fig:DHCP_diffs} represents the interleaving time distribution. The median for seeing a DHCP packet is about 3 hours.

However, on DHCP enabled networks, this drawback can be overcome and DHCP packets can be retrieved instantly, if active measures can be taken.~\footnote{Note that active probing of the IoT devices is not required.}

In a such scenario we can actively disconnecting all devices in the network. This action causes every device to renegotiate and triggers DHCP traffic. We can do this by for example running the aireplay-ng tool\cite{aireplay-ng} (part of aircrack).
We tested this technique on a LAN network and were able to retrieve the DHCP information in less than a few seconds.~\footnote{With the appropriate credentials you can use tr-69 to retrieve part of the values we previously discussed. You still can use them for classification, however, it not as robust as the method we present.}

\ignore{
However, on DHCP enabled networks, this drawback can be overcome and DHCP packets can be retrieved instantly, if active measures can be taken.~\footnote{Note that active probing of the IoT devices is not required.}

PARAMETER REQUEST LIST IS NOT AVAILABLE THROUGH TR69 :(
We propose two methods to actively retrieve DHCP packets:
\begin{itemize}
   \item Retrieve the DHCP values from the router by using the router management and control protocol. For example, the DHCP information is commonly kept in the CPE within the TR-69 data structures. TR-69 \cite{tr69} is a remote management protocol of customer-premises equipment (CPE), i.e., home-routers. 
    \item Actively disconnecting all devices in the network. This action causes every device to renegotiate and triggers DHCP traffic. We can do this by for example running the aireplay-ng tool\cite{aireplay-ng} (part of aircrack).
\end{itemize}
We implemented both techniques on a LAN network and were able to retrieve the DHCP information in less than a few seconds. 
}

\begin{figure}[t]
\centering
\psfig{file=figures/DHCP.png,width=3.5in,}
\caption{Percentage of slots that contain DHCP packets on the seen dataset} \label{fig:DHCP}

\end{figure}

\begin{figure}[t]
\centering
\psfig{file=figures/DHCP_diffs.png,width=3.5in,}
\caption{Interleaving time distribution of DHCP packets on the seen dataset} \label{fig:DHCP_diffs}
\end{figure}


In the next section, we discuss our intuition for choosing fields sources for classificaion.
In section \ref{sec:dhcp-algroithm} we discuss how we used these observations to apply a machine-learning technique and retrieved classifiers with high accuracy. 

\hl{this and the "VCI" part}
\subsection{Testing our intuition by observations}
\subsubsection{Hostname Field}

The hostname value usually contains some information about the device and the value is configured by the vendor.  For example, the hostname of Netatmo Welcome (a security camera) is 'netatmo-welcome-143453' ~\footnote{All unique identifiers in this paper are scrambled.} and the hostname for Samsung Galaxy A7 is 'Galaxy-A7-2017'. 
Note, that we are seeking for a general classifier, hence we cannot learn all the possible vendors or models, but we can make use learning all the major NoT vendors, or major OS vendors, such as Mac, Android and Microsoft.

\subsubsection{Vendor Class Identifier Field}

VCI field is mostly contains an information about the DHCP client the device make use. Some of the values we saw are: 'udhcp' - a lightweight client, 'dhcpcd' - a featureful client, common for linux/android based systems, and 'MSFT' - microsoft's DHCP client, shown exclusively for windows-based systems.

\ignoreInfocom{
\subsection{Testing our intuition by observations}
\subsubsection{Hostname Field}

The hostname value usually contains some information about the device and the value is configured by the vendor.  For example, the hostname of Netatmo Welcome (a security camera)
 is 'netatmo-welcome-143453'~\footnote{All unique identifiers in this paper are scrambled.}  and the hostname of Samsung Galaxy A7 is 'Galaxy-A7-2017'. Note, that we are seeking for a general classifier, hence we cannot learn all the possible IoT vendors, but we can learn all the major NoT vendors, or major OS vendors, such as Mac, Android and MSFT.

Sometimes the vendor or device type information is provided in the hostname itself: for example a smartphone with the hostname 'android-587f89a4a4c2eaf1' that contains the word 'android' or the TP-Link Day Night Cloud camera with the hostname 'Little Cam' that contains the word 'cam'.

\subsubsection{Vendor Class Identifier Field}

The most frequently observed identifiers of the DHCP client are as follows:
\begin{itemize}
    \item udhcp - a basic DHCP client program that is very common for IoT and embedded devices. $100\%$ of the devices that run udhcp were IoT in our dataset.
    \item dhcpcd - a feature-full DHCP client program common in Android/Linux devices. Many devices with this identifier are NoT devices; however, some IoT devices (such as Google Chromecast) also use dhcpcd. Thus we need another indicator for classifying the device. In this case, a good indication for NoT devices is the 'dhcpcd' label in VCI and an 'android' label in hostname field.
    \item MSFT - the DHCP client for every Windows device. In our dataset all the devices that use the 'MSFT' label are NoT devices.~\footnote{We are aware of 'Windows 10 IoT core'. We do not have a sample of such a device. However, after reading the descriptions and specifications we believe this product is not a 'classic IoT device'. Rather, it belongs to a grey area alongside Android smart TVs and Linux distributions mounted on RaspberryPI.}
\end{itemize}
}

\ignore{ We note that in many cases the hostname is undefined (in many of the IoT devices and in some of the NoT device). Moreover, the user can change the hostname value, and thus the value can be misleading.}


\ignore{
First, there is no convention for the hostname, that identify the type of device. Second,in many cases the  device name is related to the vendor (example XXX) and learning all the vendors, especially in IoT is not generic and not feasible. Third,  in many cases the hostname is undefined (in many of the IoT devices and in some of the NoT device). Forth, the user can change the hostname value, and thus the value  can be misleading.}

\begin{figure}[t]
\centering
\psfig{file=figures/DHCP_extracted_data.png,width=3.5in,}
\caption{Example of DHCP packet and extracted features} \label{fig:dhcp_vals}
\end{figure}

\subsection{Decision Tree Over DHCP Information} 
\label{sec:dhcp-algroithm}

Because the classification is according to words/options that appears or not in DHCP, we chose to use a decision-tree algorithm.

The hostname and VCI fields contain concatenations of words. As a first step, we extract labels (spliting words) automatically from those fields.

We split those values into labels separated by delimiters (such as: ,./\_-+). We also filter numbers. The parameter-request-list is a list of identifiers. Therefore, we add them as labels for the previous group of labels. We then construct binary vectors according those labels.
Every i-th bit in a vector represents the fact that the i-th label exists. This binary vector technique is also known as "one hot encoder". 

We train a decision-tree model \cite{PythonDecisionTreePackage} using vectors we construct according to the seen dataset.  Figure \ref{fig:dhcp_tree} visualizes the resulting tree. The decision tree contains the labels: 'dhcpcd', 'android', 'linux', '12' and '15'. Analyzing those results we find that: '12 and '15' labels derived from the parameter-request-list, 'dhcpcd' and 'linux' labels derived from the VCI field and the 'android' label can be derived from both hostname and VCI fields. Note that this list of most informative labels has chosen automatically by the decision tree algorithm.

We tested our model on the unseen dataset and achieved an F1-score of 93.33\%. For recall and precision we achieved 93.33\% and 93.33\%, respectively, on devices that use DHCP. We note that the NoT devices from CICIDS 2017 \cite{cicids2017} were configured with static DHCP, and thus the technique cannot be applied to them (22.2\% of the devices from our dataset). Our model misclassified two devices.
We tested multiple varient of this technique using subsets of the fields (hostname, VCI, parameter-request-list). In some cases we achieved lower accuracy. In others, we obtained a tree with a lot of specific labels, were not generic enough and contained words such as specific vendor names. We tried either to analyze labels from VCI field alone, we saw that all Apple devices and some IoT devices sent empty values and were misclassified. Thus, it is necessary to perform the classification on all values.

\begin{figure}[t]
\centering
\psfig{file=figures/dhcp_tree.png,width=3.5in,}
\caption{Decision tree visualization; DHCP signature-based classifier.} \label{fig:dhcp_tree}
\end{figure}

\ignore{
Those results are for devices that were connected in DHCP enabled networks.\ignore{We test our data and realized that the NoT devices from CICIDS 2017 were configured with static DHCP, therefore they did not send any DHCP data, so we skip them.}
A classifier based DHCP data has a great potential, however, it is a very limited method and can be fooled easily.
}
\ignore{
% the algorithm
In Algorithm \ref{DHCP_classifier} we demonstrate our simple signature-based classifier. vci is the observed value in the Vendor-Class-ID field, and hostname is the observed value in the hostname field. We made a list of generic defaults labels we observed in the seen dataset. The list contains the labels: '-mbp', 'android', 'bulb', 'cam', 'computer', 'dhcpcd', 'laptop', 'macbook', 'imac', 'msft', 'pc', 'phone', 'smart', 'thing', 'things' and 'udhcp'. The list 'categories' contains the categories of the decision-tree algorithm. Those values are the generic defaults labels we mention before after optimization by the decision-tree fitting procedure. In the prediction procedure we sanitize the text into a list of labels. Then, we encode the labels in a one-hot vector. Our "One-Hot" vector is based on the 'categories' list we discuss earlier. We chose this method because there is meaning whether or not each label exist in a matter of IoT/NoT classification. At last, we activate a post-trained Desition-Tree classifier model and receive a prediction. Figure \ref{fig:dhcp_tree} visualize model's decisions. Note, only labels existing in the 'categories' list will affect classification, other labels will be ignored.

\begin{algorithm}
\caption{simple DHCP signature-based classifier}\label{DHCP_classifier}
\begin{algorithmic}[1]

\State categories $= \left['udhcp', 'msft', 'android', 'macbook'
 \right]$
\State encoder = OneHotEncoder(categories)

\State
\Procedure{predict}{vci, hostname}

\State labels $\gets sanitize\_text(vci) \cup sanitize\_text(hostname)$

\State $\text{features\_vector} \gets encode(labels)$

\State \Return DesicionTreePredict($\text{features\_vector}$)

\EndProcedure
\State
\Procedure{sanitize\_text}{text}
\For {$\forall ch \in \text{text}$}
\If {ch in ",|{}[]()-+=:/\"}
\State $ch \gets$ " "
\EndIf
\EndFor
\State \Return text.split(" ")
\EndProcedure
\State
\Procedure{encode}{labels}
\State \Return encoder.transform(labels)

\EndProcedure

\end{algorithmic}
\end{algorithm}
}

\ignore{
\begin {table*}[ht]
\begin{center}
\resizebox{\linewidth}{!}
{
\begin{tabular}{|l||l|l|l|l|l|l| }
\hline
Protocol	& Classification Latency &	Grade: F1-Score & Accuracy: Recall & Accuracy: Precision & Efficiency & Architecture \\
\hline
\hline
DHCP & Long & 99.52\% & 100\% & 99.06\% & Limited: DPI required & LAN or TR-69\\

\hline
\end{tabular}}

\vskip 6pt
\caption{Rule-based classifier over DHCP data results \vspace{-0.5cm}} \label{tab:dhcp_results} 
\end{center}
\end {table*}
}


==> sections/background.tex <==
\section{Background: IoT and Security mechanism}

There are three possible deployment options of IoT. 

As  far  as  we  are  aware  of,  this  is  the  only  solution  that  isdeployed at the network-level. There are another three possibledeployment locations for such appliances: (i) on the IoT deviceitself,  i)

\begin{enumerate}
    \item By  an  additional  device  on  the  home network.
     Some  startups  and  companies  (such  as Cujo,  Dojo,  RatTrap,  F-secure,  and  Trend  Micro)  have  tried  this option. 
     \item  In the Customer Premise Equipment (CPE)  - I.e., the home router. Recently, there is a recent shift in Industry to this option (e.g.,  ARRIS  and  D-LINK  CPE  with McAfee solution , ASUS CPE with Trend Micro Solution, and more).
     \item Solution at the ISP (Internet Service Provider) level -  ISP can provide IoT security as a service to  its  customers. This solution requires configuring the CPE using TR 69 protocol, in order to colored all the flows that coming from the same device in the same color. 
     
\end{enumerate}


==> sections/features.tex <==
\section{Simple Classifier on Traffic Features}
In this section, we propose a classifier on traffic features, where the features are numeric. We begin by exploring the different possible features we checked and their motivation. We then  construct a simple classifier. It turns out that the a classifier that work only a small subsets of features achieves good results. 
In section \ref{ } we explain the feature selection and the intuition behind the features.
We then, explain in section \ref{ }   how we construct the optimal feature sets. Finally, in section \ref{ } we explain the resulted classifier and presnet expermintal results of its accuracy.  



\begin {table*}[ht]
\begin{center}
\resizebox{\linewidth}{!}
{
\begin{tabular}{|l||l|l| }
\hline
Feature name	& Feature description &	f1-score \\
\hline
\hline

window size &	maximum TCP window size &	$0.942$ \\
\# unique DNS  &	number of unique DNS queries &	$0.845$ \\
\# remote ip &	number of unique interacted  endpoints of remote IPs  &	$0.829$ \\
\# dns req &	number of DNS queries &	$0.738$ \\
\# ports &	number of unique outgoing ports & 	$0.658$ \\
bandwidth	& bandwidth (in bytes) of outgoing traffic  & 	$0.601$  \\
pckt count	& number of outgoing packets & 	$0.588$ \\
tcpts &	 linear-least-square error for TCP timestamp value &	$0.582$ \\
interleaving deviations & standard deviation of interleaving time for outgoing packets  &	$0.576$ \\
tcp/udp ratio & ratio between the number of TCP to UDP  packets &	$0.548$ \\
avg ttl	 &  average of the  TTL field in outgoing IP packets & $0.481$ \\
avg ua	& average length of user-agent field in http requests & $0.461$ \\

\hline
\end{tabular}}

\vskip 6pt
\caption{List of features collected for each device and their classification score. The score was calculated using F1-score on 'seen' dataset (5-fold cross-validation) using each feature alone, for a time slots of 10 minutes.} \label{tab:features} 
\end{center}
\end {table*}


In Table \ref{tab:features} we list possible features, we have checked. Our main intuition was that there is an inherent difference between IoT and NoT. IoT is not as a general computer. IoT has more expected network traffic rate and patterns, connects to limited endpoints (mostly vendor cloud servers). IoT can be characterized by more monotonic processing intensity and has lower resources (CPU and memory).

We give here an  explanation on some of the features, and the intuition, why we thought it can separate between IoT to NoT device. We begin with features with higher F1-score, when checking the F1-score of each feature separately.  

\subsubsection{TCP window size}
IoT devices are not equipped as NoT devices. This can be caused by the specific purpose of the devices and the need to maintain low costs. Therefore, we expect IoT devices to suggest lower buffer size for TCP stack \cite{C.GomezJ.CrowcroftScharf2018}. This buffer size can be emerged in the window size field as part of the TCP layer. Figure \ref{fig:winds_cdf} visualize the IoT's window size values CDF versus NoT's values reverse-CDF. This comparison shows the separability over this feature. This feature has great availability, visibility and is unencrypted  . Most of our devices (XXX\%), had TCP traffic in their time slots. 

\subsubsection{number of unique DNS request and number of unique remote IPs}
 
 IoT commonly interact with a-small set of endpoints (usually cloud servers), this impact also the set of domains that it needs to resolve, in order to receive the IP's endpoint.  Figure \ref{fig:udns_cdf} visualize the IoT's number of unique dns domain values CDF versus NoT's values.   The availability of DNS  Figure \ref{fig:DNS_per} is high enough for classification. Moreover, in DNS context, no data is data. Lake of DNS traffic can tell us information about the device. At last, DNS is also unencrypted (until adaptation of DNS over TLS). We note that the fact that IoTs usually have small number of unique DNS request was observed also in \cite{}.
 We can also use the IP information, and capture  the number of unique remote-IPs (remote endpoints) of each device.   We note that there is a difference between the number of unique DNS and the number of unique remote IP. Since we capture the traffic in some slot, i.e., in the middle of the device operation,  we might not capture the DNS queries that resolve the IPs. 
 
\ignore{
\subsubsection{Packet Intensity}
As feature candidates we chose packet's length, rate and intensity (sum per slot). The advantages choosing those features is by their visibility; can be probed from CPE as from ISP locations (can be measured at IP layer either). They are very available, they commonly used. And they are unencrypted.

\subsubsection{Remote IP}
IoT devices designed for specific assignments, therefore, they should connect mainly to their vendor's C\&C and/or cloud server. in contrast to NoT devices which is connects to various servers. From IP layer we extract the remote-IP values and count the unique remote-IPs for each device. IP layer is available, visible and unencrypted.
}

\subsubsection{HTTP User-Agent length}
\label{subsec:UA}

 User agent is being send during HTTP requests, and it  contains a short description of the properties of the requesting device. For NoT devices, this parameter has  usually longer length, since  this parameter describes properties which is  relevant only for Not devices, such as screen size, OS language and browser. 

We made an analysis on our devices data set (see Section \ref{sec:methodology} for details on the data set) for how frequent requests with User agent are. Figure \ref{fig:UA_per} shows the presence of HTTP requests in various time slots, and Figure shows \ref{fig:UA_diffs} the interleaving time distribution between HTTP requests. The results show that the classification latency is  high, the chance to find an User Agent value sent by a IoT device in a slot of 20 minutes is about 25\%. We note that unlike the DHCP client information, the User agent is an information that was sent to the endpoints, and hence it is not stored at the home-router and thus cannot be actively retrieved. 

Using User Agent, for classification as was suggested at \cite{Meidan2017}, is not applicable to our requirement,  due  to  the  fact  that  it  has  high latency classification time, some devices do not send it and is increasingly  being  transferred  on  encrypted  traffic  (a blackout  of  about  50\%  of  IoT  devices).

Nonetheless, we use the User agent length, as one of the features for ML traffic features classification, however as it shown in Section \cite{}, it was not picked by the algorithm. 

\begin{figure}[t]
\centering
\psfig{file=figures/UA_per.png,width=3.5in,}
\caption{Percentage of slots that contains plain-text User-Agent field} \label{fig:UA_per}
\end{figure}


\begin{figure}[t]
\centering
\psfig{file=figures/UA_diffs.png,width=3.5in,}
\caption{Interleaving time distribution of packets with plain-text User-Agent field} \label{fig:UA_diffs}
\end{figure}

\ignore{
As we mention before, UA field contains a short description of the target system. It contains information about the system, platform, browser, screen resolution and language. Most of these parameters are not relevant for IoT devices. Therefore, IoT UA may be shorter than NoT UA. We extract UA lengths for each device in each slot and made an average. HTTP is visible from different probing locations; however, it is not very common (not as IP or even DNS) and visible only on unsecured connections.}



\begin{figure}[t]
\centering
\psfig{file=figures/max_winds_sd_1200.png,width=3.5in,}
\caption{Comparison between IoT to NoT window size values} \label{fig:winds_cdf}
\end{figure}

\begin{figure}[t]
\centering
\psfig{file=figures/TCPTS_per.png,width=3.5in,}
\caption{Percentage of slots that contains TCP-Timestamp field} \label{fig:TCPTS_per}
\end{figure}

\subsubsection{TCP Timestamp}
I DO NOT UNDERSTAND ANYTHING FROM THIS PARAGRAPH. ESPECIALLY I CANNOT SEE THIS PARAMETER IN THE TABLE OF FEATURES !!!!
TCP timestamp is a TCP option being used to measure RTT. As suggested in RFC 1323 \cite{Jacobson1992} TCPTS is incremented according to a 'virtual clock' that depends on the device's CPU. This clock has a bias that emerge on TCP packets. We suggested that more monotonic CPU processing intensity results with a higher bias for this clock. Therefore, we extract the arrival time and TCPTS values from each TCP packet contained this parameter. For each device we calculate Linear least square on those arrays. We collect the error as a feature. Figure \ref{fig:TCPTS_per} shows the separation between IoT to NoT given TCPTS error. THE FIGURE DOESNOT SHOW IT!!!!  IoT plot showing as a CDF, when NoT plot showing as a reverse-CDF. We did not dig into this area any further, there is more work to be done in order to better understand this symptom over various scenarios (working on battery, energy saving mode, data saver, etc...).

\begin{figure}[t]
\centering
\psfig{file=figures/DNS_per.png,width=3.5in,}
\caption{Percentage of slots that contains DNS packets} \label{fig:DNS_per}
\end{figure}

\ignore{
\subsubsection{DNS domains \& unique domains}
While IoT purposed to interact with specific server, there should be a different behavior onto DNS traffic. Figure \ref{fig:udns_cdf} as above, visualize the separability of this feature. In each slot we collect the number of queries and unique queries requested by each device. We use this data as features. DNS traffic is visible and can be measured from remote locations. DNS protocol is not as available as ethernet, IP or TCP, but as Figure \ref{fig:DNS_per} suggest, its availability is high enough for classification. Moreover, in DNS context, no data is data. Lake of DNS traffic can tell us information about the device. At last, DNS is either unencrypted (until adaptation of DNS over TLS).
}

\begin{figure}[t]
\centering
\psfig{file=figures/udns_sd_1200.png,width=3.5in,}
\caption{Comparison between IoT to NoT unique DNS queries} \label{fig:udns_cdf}
\end{figure}


==> sections/methods.tex <==
\hl{from here until the  'TCP window size' subsection}
\section{Simple Classifier on Traffic Features}
In this section, we propose a classifier that operates on traffic features, where the features are numeric. We begin by exploring the different possible features and their motivation. We then construct a simple classifier. It turns out that a classifier that works only on a small subset of features achieves good results. 
In Section \ref{seq:feature_selection} we explain the feature selection and the intuition behind the features.
We then explain in Section \ref{seq:optimal_set} how we construct the optimal feature sets. Finally, in Section \ref{seq:exper_res} we explain the resulting classifier and present experimental results that demonstrate its accuracy on the unseen data set.

\subsection{Feature Selection}
\label{seq:feature_selection}

Our main intuition was that there is an inherent difference between IoT and NoT devices. Unlike a general-purpose computer,  an IoT has a higher expected network traffic rate and more patterns, and it connects to limited endpoints (mostly vendor cloud servers). IoT devices can be characterized by a more monotonic processing intensity and lower resource usage (CPU and memory).

We have tested many features from all common protocols (such as: relations between outgoing packets, IP, TCP, DNS, HTTP, ..). In order to check the separability of each feature, we first had to normalize the seen traffic, such that the same number of samples was taken from each device. This helped us deal with the big differences in recording time, where some devices were recorded for weeks and some for hours. In order to represent a wide range of scenarios, we chose representative samples according to bandwidth (low, medium and high).
Then, we analyzed those sets (IoT vs NoT) using statistical tools (such as Welch's t-test, ROC curve and AUC calculation \cite{Welch2008, Fawcett2006}) in order to determine the separation potential for each feature. Using those measures, we filtered our entire feature set into an informative, small set of 10 features, each calculated per time slot, as shown in Table \ref{tab:features}.

\ignoreInfocom{
We checked many features (see Table \ref{tab:raw_features}). In order to check the separability of each feature, we first had to normalize the seen traffic, such that the same number of samples was taken from each device. This helped us deal with the big differences in recording time, where some devices were recorded for weeks and some for hours. In order to represent a wide range of scenarios, we chose representative samples according to bandwidth (low, medium and high).
Then, we analyzed those sets (IoT vs NoT) using statistical tools (such as Welch's t-test, ROC curve and AUC calculation \cite{Welch2008, Fawcett2006}) in order to determine the separation potential for each feature. Using those measures, we filtered our entire feature set into an informative, small set of 12 features, each calculated per time slot, as shown in Table \ref{tab:features}.

\begin {table*}[ht]
\begin{center}
\resizebox{\linewidth}{!}
{
\begin{tabular}{|l||l| }
\hline
Layer	& Feature description \\
\hline
\hline

Link-Layer & Number of outgoing packets                                         \\
Link-Layer & Bandwidth (in bytes) of outgoing traffic                           \\
Link-Layer & Average (in bytes) of packets length                               \\
Link-Layer & Average of interleaving time for outgoing packets                  \\
Link-Layer & Standard deviation of interleaving time for outgoing packets       \\
IP & Number of unique interacted endpoints of remote IPs                        \\
IP & Average of the TTL value in outgoing IP packets                            \\
IP & Average of the header length value in outgoing IP packets   \\
IP & Maximum of the header length value in outgoing IP packets   \\
IP & Minimum of the header length value in outgoing IP packets   \\
IP & Count of unique header length values in outgoing IP packets \\
IP & Number of unique outgoing ports                                            \\
IP & Ratio between the number of TCP to UDP  packets                            \\
IP & Number of unique interacted endpoints of remote End-Points (IP $\times$ Ports)    \\
TCP & Maximum TCP window size                                                   \\
TCP & Mean TCP window size                                                      \\
TCP & Minimum TCP window size                                                   \\
TCP & Count of unique TCP window size values                                   \\
TCP & Linear-least-square error for TCP timestamp value                         \\
DNS & Number of unique DNS queries                                              \\
DNS & Number of DNS queries                                                     \\
HTTP & Average length of user-agent field in http requests                      \\

\hline
\end{tabular}}

\vskip 6pt
\caption{List of raw features tested.} \label{tab:raw_features} 
\end{center}
\end {table*}

}

The last column shows the F1-score for the 'seen' dataset. The classification latency was 10 minutes. We calculated the F1-score using 5-fold cross-validation, a common technique in machine learning, to choose features with no over-fitting. Our 5-fold cross-validation method randomly splits the devices in the dataset into 5 \textbf{independent sets} of train (80\%) and test (20\%). Note that no device appears in more than one test set.  Every test was run 5 times, once for each fold, and the results were averaged. We focused on the set of features whose F1-score was above 0.5.

For features that depend on information that appears only from time to time in the traffic (e.g., TCP timestamp or user-agent), Not all slots contained values. Thus, we filled the missing values with average values we learned for those features from the 'seen' dataset.  Therefore, a low F1-score may also indicate that this feature does not appear in most slots. 

\begin {table*}[ht]
\begin{center}
\resizebox{\linewidth}{!}
{
\begin{tabular}{|l||l|l| }
\hline
Feature name	& Feature description &	F1-score \\
\hline
\hline

window size &	maximum TCP window size &	$0.942$ \\
\# unique DNS  &	number of unique DNS queries &	$0.845$ \\
\# remote ip &	number of unique interacted  endpoints of remote IPs  &	$0.829$ \\
\# dns req &	number of DNS queries &	$0.738$ \\
\# ports &	number of unique outgoing ports & 	$0.658$ \\
bandwidth	& bandwidth (in bytes) of outgoing traffic  & 	$0.601$  \\
pckt count	& number of outgoing packets & 	$0.588$ \\
tcp ts deviation &	 linear-least-square error for TCP timestamp value &	$0.582$ \\
interleaving deviations & standard deviation of interleaving time for outgoing packets  &	$0.576$ \\
tcp/udp ratio & ratio between the number of TCP to UDP  packets &	$0.548$ \\
%avg ttl	 &  average of the  TTL field in outgoing IP packets & $0.481$ \\
%avg ua	& average length of user-agent field in http requests & $0.461$ \\

\hline
\end{tabular}}

\vskip 6pt
\caption{List of features collected for each device and their F1 classification score. The F1-score was calculated on the 'seen' dataset (5-fold cross-validation) using each feature alone, for a time slot of 10 minutes.} \label{tab:features} 
\end{center}
\end {table*}

We next explain some of the most informative features, and our intuition as to why we thought these features would successfully distinguish between IoT and NoT devices. We begin with features with a higher F1-score, when checking the F1-score of each feature separately.


\subsubsection{TCP window size}
IoT devices are less fully equipped than NoT devices. This might be due to the specific purpose of the devices and the need to maintain low costs. We therefore expect that IoT devices have a smaller buffer size for the TCP stack \cite{C.GomezJ.CrowcroftScharf2018}. The size of the TCP Receive Window is transferred to the connection endpoint using the window size value field of the TCP header. Figure \ref{fig:winds_cdf} compares the CDF of the IoT window size values to the reverse-CDF of the NoT window size values. This comparison shows the separability over this feature. This feature is highly available, visible and unencrypted. All of our devices had TCP traffic in their time slots. 

\subsubsection{Number of Unique DNS Requests and Number of Unique Remote IPs}
 
IoTs commonly interact with a small set of endpoints (usually cloud servers), which also influences the set of domains that it needs to resolve in order to receive the IP's endpoint. Figure \ref{fig:udns_cdf} compares the CDF of the number of unique DNS queries of IoT devices to the reverse-CDF for NoT devices. This is a common technique for visualizing the separability of a feature. Moreover, if there is no DNS traffic, this is also data, and the value of the feature for that slot will be zero.

We note that the small number of unique DNS requests in IoT devices was also observed in \cite{Sivanathan2017}.
We can also use the IP information, and capture the number of unique remote-IPs (remote endpoints) of each device. We further note that the number of unique DNS requests and the number of unique remote IPs is not the same. Since we capture the traffic in some slot, i.e., in the middle of the device operation, we might not capture the DNS queries that resolve the IPs due to DNS caching.
 
\ignore{
\subsubsection{Packet Intensity}
As feature candidates we chose packet's length, rate and intensity (sum per slot). The advantages choosing those features is by their visibility; can be probed from CPE as from ISP locations (can be measured at IP layer either). They are very available, they commonly used. And they are unencrypted.

\subsubsection{Remote IP}
IoT devices designed for specific assignments, therefore, they should connect mainly to their vendor's C\&C and/or cloud server. in contrast to NoT devices which is connects to various servers. From IP layer we extract the remote-IP values and count the unique remote-IPs for each device. IP layer is available, visible and unencrypted.

}
\subsubsection{IP Time-to-Live}
IP's field of time-to-live is a well-known indicator that can assist OS fingerprinting. This field is very attractive due to its availability and visibility. 


\subsubsection{HTTP User-Agent Length}
\label{subsec:UA}

The user-agent parameter is sent during HTTP requests, and it contains a short description of the properties of the requesting device. For NoT devices, this parameter is usually longer, since it describes properties relevant only for NoT devices, such as screen size, OS language and browser.

We analyzed our device dataset (see Section \ref{sec:methodology} for details on the dataset) to determine the frequency of requests with the user-agent parameter. Figure \ref{fig:UA_per} shows HTTP requests in various time slots, and Figure  \ref{fig:UA_diffs} shows the interleaving time distribution between HTTP requests. The results show that the classification latency is high, and the chance to find a user-agent value sent by a IoT device in a slot of 20 minutes is about 25\%. We note that unlike the DHCP client information, the user-agent information was sent to the endpoints; hence it is not needed/stored at the home-router and thus cannot be actively retrieved. 

The authors of \cite{Meidan2017} suggested that the user-agent value could be used for classification, but it does not meet our requirements due to its high-latency classification time. Moreover, some devices do not send this value, or transfer it on encrypted channels (about  50\%  of our IoT devices).

\ignoreInfocom{
Nonetheless, we use the user-agent length parameter for traffic feature classification. However, as we will show in Section \ref{seq:optimal_set}, this feature was not chosen by the logistic-regression algorithm.
}

\begin{figure}[t]
\centering
\psfig{file=figures/UA_per.png,width=3.5in,}
\caption{Percentage of slots that contain plain-text user-agent field, seen dataset)} \label{fig:UA_per}
\end{figure}


\begin{figure}[t]
\centering
\psfig{file=figures/UA_diffs.png,width=3.5in,}
\caption{Interleaving time distribution of packets with plain-text user-agent field, seen dataset} \label{fig:UA_diffs}
\end{figure}


\begin{figure}[t]
\centering
\psfig{file=figures/max_winds_sd_1200.png,width=3.5in,}
\caption{The values of maximum TCP window size in IoT devices (presented as CDF) and NoT devices (presented as Reverse-CDF), seen dataset }
\label{fig:winds_cdf}
\end{figure}

\begin{figure}[t]
\centering
\psfig{file=figures/TCPTS_per.png,width=3.5in,}
\caption{Percentage of slots that contain TCP-Timestamp field, seen dataset} \label{fig:TCPTS_per}
\end{figure}

\subsubsection{TCP Timestamp Deviation}
The TCP timestamp is a TCP option used to measure RTT. As suggested in RFC 1323 \cite{Jacobson1992}, TCPTS is incremented according to a 'virtual clock' that depends on the device's CPU. This clock has a bias that emerges on TCP packets. Our guess was that less monotonic CPU processing intensity would result in a greater bias for this clock. Thus we assumed that greater bias would be observed for NoT devices than IoT devices. Therefore, we extract the arrival time and TCPTS values from each TCP packet containing this parameter. For each device we calculate linear least square error  on those values. We collect the error as a feature. Figure \ref{fig:TCPTS_per} shows the availability of this optional field in our seen dataset.  

\ignore{
\begin{figure}[t]
\centering
\psfig{file=figures/DNS_per.png,width=3.5in,}
\caption{Percentage of slots that contain DNS packets} \label{fig:DNS_per}
\end{figure}}

\begin{figure}[t]
\centering
\psfig{file=figures/udns_sd_1200.png,width=3.5in,}
\caption{The number of unique DNS queries in IoT devices (presented as CDF) and NoT devices (presented as Reverse-CDF)} \label{fig:udns_cdf}
\end{figure}


\begin{algorithm}
\caption{The Classification Algorithm}\label{main_classifier}
\begin{algorithmic}[1]
\Procedure{predict}{$\vec{x}$}
\State \text{learned parameters:} $\vec{\theta}, (\vec{\mu}, \vec{\sigma}), \vec{\text{def}}$
\State $x \gets $imputation($\vec{x}, \vec{def}$)
\State $x \gets $normalize($\vec{x}, (\vec{\mu}, \vec{\sigma})$)
\State $prediction \gets \text{sign}( (1, \vec{x}) \cdot \vec{\theta} )$
\State \If {$prediction \leq 0$}
\State {\Return \text{NoT}}
\Else 
\State \Return \text{IoT}
\EndIf
\EndProcedure
\State
\State

\Procedure{imputation}{$\vec{x}, \vec{def}$}
\For {$i \gets 1$ to $||\vec{x}||$}
\If {$x_i$ is undefined}
\State {$x_i \gets $ def$_i$}
\EndIf
\EndFor
\State \Return $\vec{x}$
\EndProcedure
\State
\State

\Procedure{normalize}{$\vec{x}, (\vec{\mu}, \vec{\sigma})$}
\For {$i \gets 1$ to $||\vec{x}||$}
\State {$x_i \gets (x_i - {\mu}_i) / \sigma_i$}
\EndFor
\State \Return $\vec{x}$
\EndProcedure
\end{algorithmic}
\end{algorithm}

\subsection{Constructing the Optimal Feature Set}
\label{seq:optimal_set}

Our classifier uses sklearn's StandardScaler function \cite{standard_scaler} in order to standardize feature values and relies on the logistic regression algorithm \cite{Regression1978} when applying classification. In order to test incoming traffic against the classifier, we apply Algorithm \ref{main_classifier} on an extracted feature set $x$. $\theta$ are the trained coefficients for the logistic regression algorithm, $\mu$ and $\sigma$ are vectors of the trained mean and scale for the standard scaling for each feature type in the sets, and $def$ is a vector used to impute values for each feature type in case of missing values.  $\mu, \sigma$ and $def$ are general vectors for IoT and NoT.

\hl{abducted from the end of this section}
Performance wise, implementing the classifier on traffic features requires finding the number of distinct elements (of the number of unique dns queries and the number of remote IPs). Note, however, that if the number of distinct elements is small, the naive solution would be to restore the last $x+1$ unique elements seen.
 Since the threshold of the number of unique elements is small, this is a practical solution. One may also apply algorithms that approximate the number of distinct elements, such as \cite{superspreaders:NDSS2005, Bandi:ICDCS2007,Locher:spaa2011}.

In order to construct a machine learning model, we must choose a combination of features that optimizes prediction rates. The challenge is even more difficult because we need to find the best number of features in addition to the best features themselves. Note that an optimal set of features for classification latency of 5 minutes is not necessarily an optimal set for any other classification latency. Therefore, we need to learn optimal sets for each classification latency.
To do so, we apply our learning using 5-fold cross-validation, as proposed in Section \ref{seq:feature_selection}

To learn the optimal number of features and the optimal features themselves, we used a greedy algorithm. We found the feature with the highest F1-score, adding it to our feature vector. Then we tested every other feature appended to the feature vector, choosing the group with the highest F1-score. We computed this score for each classification latency. Our goal was not only to optimize the F1-score for each latency but also the number of selected features. We used a parameter $\alpha$ as a threshold in order to prefer a smaller vector size over a larger one with a tiny performance increase. In our case, we chose $\alpha$ to be $1\%$.
The equations below present our feature selection algorithm. $F$ is the feature pool, $t$ is the classification latency, and $i$ is the vector V size. $V_t(i)$ is the optimal i-sized vector for t classification latency. $V_t$ is the optimal vector of features for t classification latency.

\begin{align}
&\forall f \in F \;\;\;\;\;\; V_t(1)=\argmax_f(\text{F1-score}(f))\\
&\forall f \in F \;\;\;\;\;\; V_t(i)=\argmax_f(\text{F1-score}(V_t(i-1)\cup{f}))
\end{align}

$$\forall i = 0..||V_t||$$ 
\begin{equation}
V_t =
\begin{cases}
V_t(i) & \text{if } \frac{V_t(i+1)-V_t (i)}{1-V_t(i)} < \alpha \\
V_t(i+1) & \text{otherwise}
\end{cases}
\end{equation}

For all the possible classification latencies, the feature set size did not exceed 4.

Table \ref{tab:Best_features} shows the optimal combinations and their averaged F1-score over the 5-fold cross-validation for each classification latency (on the 'seen' dataset). 

\hl{some changes in this paragraph}
For testing versus cross-validation, we did not choose samples from the dataset. We used the entire dataset for testing. Using all the data better reflects the targeted 'outside' environment. The technique is to test each device separately, exporting an average of its successful prediction rate and later averaging the scores of all the devices. This technique allows us to test each device in as many situations as we can. As at the same time, we avoid any bias caused by the difference in the online periods of the devices.

\begin {table*}[ht]
\begin{center}
\resizebox{\linewidth}{!}
{
\begin{tabular}{|l||l|l| }
\hline
Classification Latency & F1-Score & Feature set \\
\hline
\hline
1 min & 89.52\% & window size, \# unique DNS req, tcp/udp ratio, pckt count \\
5 min & 89.67\% & window size, \# unique DNS req, \# remote IP \\
10 min & 93.39\% & window size, \# unique DNS req, \# remote IP, interleaving deviations \\
20 min & 95.54\% & window size, \# unique DNS req, \# remote IP \\

\hline
\end{tabular}}

\vskip 6pt
\caption{Best feature sets for each classification latency with the F1-Score over cross-validation data (seen dataset)} \label{tab:Best_features} 
\end{center}
\end {table*}


\subsection{Experimental Results}
\label{seq:exper_res}

After training our models using the optimal combinations, we validate them against the 'unseen' dataset. Table \ref{tab:final_results} shows that we received a good score for 1 minute and very high scores from 5 minutes and above. As we did in the cross-validation scenario, we also take here all the time-slots and average the results per device. As expected, adding information (longer classification latency) to the model usually increases the success rate. In addition, we made an analysis of classification performance per device, represented at table \ref{tab:after_results}. In this table we can saw that the high accuaracy is distributed between the devices, thus there is a high classification rate for each device.

\ignoreInfocom{
Moreover, the high recall in contrast to the relatively low precision indicates that most of the errors in our models are False-positive. False-positive errors are 'better' errors due to the vulnerability of IoT devices.
}

\begin {table}[ht]
\begin{center}
\resizebox{\linewidth}{!}
{
\begin{tabular}{|l||l| }
\hline
Device & accuracy for 10 min \\
\hline
\hline
Dell Laptop win10           &  100\%  \\
ipad                        &  100\%  \\
MAC                         &  100\%  \\
Mac laptop                  &  100\%  \\
omri's ubuntu               &  100\%  \\
samsung s5                  &  100\%  \\
some xiaomi                 &  100\%  \\
testbed09                   &  100\%  \\
testbed13                   &  100\%  \\
xiaomi A2                   &  100\%  \\
Bezeq smarthome             &  100\%  \\
Foscam                      &  100\%  \\
Google Home mini            &  100\%  \\
Google Mini                 &  100\%  \\
iRobot                      &  100\%  \\
lifiLab                     &  100\%  \\
Motorola Hubble             &  100\%  \\
NestCam                     &  100\%  \\
Provision ISR               &  100\%  \\
RENPHO Humidifier           &  100\%  \\
Ring Doorbell               &  100\%  \\
samsung smart home camera   &  100\%  \\
smartHub                    &  100\%  \\
TPLink SmartPlug            &  100\%  \\
Wyze Cam                    &  100\%  \\
Ubuntu 14.4 32B             &  97.95\%  \\
Ubuntu 14.4 64B             &  97.95\%  \\
Windows Laptop              &  97.05\%  \\
Ubuntu 16.4 64B             &  95.91\%  \\
Ubuntu 16.4 32B             &  91.83\%  \\
Win 8.1 64B                 &  91.66\%  \\
Apple iPhone                &  91.07\%  \\
android samsung             &  90.90\%  \\
Win 10 pro 32B              &  89.79\%  \\
Win 7 Pro 64B               &  81.63\%  \\

\hline
\end{tabular}}

\vskip 6pt
\caption{Concluding results per device for 10 minutes classifier} \label{tab:after_results}
\end{center}
\end {table}

\ignoreInfocom{
\begin {table*}[ht]
\begin{center}
\resizebox{\linewidth}{!}
{
\begin{tabular}{|l||l|l|l|l|l| }
\hline
Device & class & accuracy for 1 min & accuracy for 5 min & accuracy for 10 min & accuracy for 20 min \\
\hline
\hline

android samsung & NoT &   0.845588235   &   0.974358974   &   0.909090909   &   0.96 \\
Apple iPhone    & NoT &   0.678111588   &   0.747474747   &   0.910714286   &   1 \\
Dell Laptop win10   & NoT &   0.8125   &   1   &   1   &   1 \\
Apple Ipad    & NoT &   0.956521739   &   1   &   1   &   0.966666667 \\
Macbook & NoT &   0.986577181   &   1   &   1   &   1 \\
Mac laptop  & NoT &   1   &   1   &   1   &   0.733333333 \\
Ubuntu PC  & NoT &   0.03030303   &   0.714285714   &   1   &   1 \\
samsung s5  & NoT &   0.909090909   &   0.8   &   1   &   1 \\
xiaomi smartphone & NoT &   0.718309859   &   0.941176471   &   1   &   1 \\
testbed09   & NoT &   1   &   1   &   1   &   0.96 \\
testbed13   & NoT &   1   &   1   &   1   &   0.5 \\   
Ubuntu 14.4 32B & NoT &   0.448687351   &   0.835051546   &   0.979591837   &   1 \\
Ubuntu 14.4 64B & NoT &   0.458139535   &   0.918367347   &   0.979591837   &   0.96 \\
Ubuntu 16.4 32B & NoT &   0.546511628   &   0.835051546   &   0.918367347   &   0.942857143 \\
Ubuntu 16.4 64B & NoT &   0.516483516   &   0.846938776   &   0.959183673   &   0.92 \\
Win 10 pro 32B  & NoT &   0.606557377   &   0.793814433   &   0.897959184   &   1 \\
Win 7 Pro 64B   & NoT &   0.604113111   &   0.760416667   &   0.816326531   &   0.96 \\
Win 8.1 64B & NoT &   0.757575758   &   0.882978723   &   0.916666667   &   0.96 \\
Windows Laptop  & NoT &   0.71086262   &   0.984496124   &   0.970588235   &   1 \\
xiaomi A2   & NoT &   1   &   1   &   1   &   1 \\
Piper camera & IoT &   0.890142715   &   0.999382462   &   1   &   1 \\
Foscam  & IoT &   1   &   1   &   1   &   1 \\
Google Home mini    & IoT &   0.995260664   &   0.988235294   &   1   &   1 \\
Google Home Mini & IoT &   0.998080614   &   0.995744681   &   1   &   1 \\
iRobot  & IoT &   1   &   1   &   1   &   1 \\
LifiLab & IoT &   1   &   1   &   1   &   1 \\
Motorola Hubble & IoT &   1   &   1   &   1   &   1 \\
NestCam & IoT &   0.936294479   &   1   &   1   &   1 \\
Provision ISR   & IoT &   0.958333333   &   1   &   1   &   1 \\
RENPHO Humidifier   & IoT &   1   &   1   &   1   &   1 \\
Ring Doorbell   & IoT &   0.866666667   &   1   &   1   &   1 \\
samsung smart home camera   & IoT &   1   &   1   &   1   &   1 \\
Samsung SmartHub    & IoT &   0.998763906   &   1   &   1   &   1 \\
TPLink SmartPlug    & IoT &   0.937169701   &   1   &   1   &   1 \\
Wyze Cam    & IoT &   0.956602031   &   0.995951417   &   1   &   1 \\

\hline
\end{tabular}}

\vskip 6pt
\caption{Concluding results per device of both of the classifiers} \label{tab:after_results}
\end{center}
\end {table*}
}
\begin {table*}[ht]
\begin{center}
\resizebox{\linewidth}{!}
{
\begin{tabular}{|l||l|l|l|l|l| }
\hline
Classifier	& Classification Latency &	 F1-Score & Recall &  Precision & Efficiency\\
\hline
\hline
DHCP & Long unless special permissions & 96.55\% & 93.33\% & 100\% &  DPI required\\
Traffic Features & 1 min & 84.75\% & 96.95\% & 75.27\%  & Counters\\
Traffic Features & 5 min & 94.31\% & 99.55\% & 89.59\%  & Counters\\
Traffic Features & 10 min & 97.85\% & 99.97\% & 95.81\% & Counters\\
Traffic Features & 20 min & 96.76\% & 100\% & 93.73\%   & Counters\\
\hline
\end{tabular}}

\vskip 6pt
\caption{Concluding results of both of the classifiers over the unseen dataset} \label{tab:dhcp_results}\label{tab:final_results} 
\end{center}
\end {table*}

\ignoreInfocom{
We give here an example of the operation of our classifier. For 5 minutes, our model works for three features: window size, Remote IP and unique DNS. The learning phase outputs:
\begin{align*}
def & = \left[ 35687.5, 9.75, 3.0 \right] \\
\mu & = \left[ 31621.863, 15.404, 8.636 \right] \\
\sigma & = \left[ 28760.610, 22.074, 17.872 \right] \\
\theta& = \left[ -0.128, -2.288, -2.079, -1.482 \right]
\end{align*}
A sample of a maximum window size of 12000 bytes, 5 unique remote IP endpoints and 3 unique DNS queries will be processed as follows:
\begin{align*}
X & = \left[ 12000, 5, 3 \right] \\
RegulatedX & \gets \left[-0.682, -0.471, -0.315 \right] \\
prediction & = 2.879
\end{align*}

When the prediction is above 0, it is interpreted as an IoT classified device.
}
